Towards Transparent Interactive Semantic Parsing via Step-by-Step Correction

Existing studies on semantic parsing focus primarily on mapping a natural-language utterance to a corresponding logical form in one turn. However, because natural language can contain a great deal of ambiguity and variability, this is a difficult challenge. In this work, we investigate an interactive semantic parsing framework that explains the predicted logical form step by step in natural language and enables the user to make corrections through natural-language feedback for individual steps. We focus on question answering over knowledge bases (KBQA) as an instantiation of our framework, aiming to increase the transparency of the parsing process and help the user appropriately trust the final answer. To do so, we construct INSPIRED, a crowdsourced dialogue dataset derived from the ComplexWebQuestions dataset. Our experiments show that the interactive framework with human feedback has the potential to greatly improve overall parse accuracy. Furthermore, we develop a pipeline for dialogue simulation to evaluate our framework w.r.t. a variety of state-of-the-art KBQA models without involving further crowdsourcing effort. The results demonstrate that our interactive semantic parsing framework promises to be effective across such models.

==> methodology.tex <==

\section{\hs{Framework}}
\label{methodology}



 In this work, we seek to design an interactive semantic parsing framework to correct initial parses produced by KBQA semantic parsers via step-by-step user interaction. Formally, given a complex question $Q$, a knowledge base $B$, a predicted parse from a base parser $P'$, and natural-language feedback $F$ from the user, the goal is to derive a corrected parse $P$. 
 
 
 To construct such a framework, as shown in Figure~\ref{fig:full_process}, we (1) first break down the initial parse predicted by a base parser into sub-LFs (Logical Form Decomposition), (2) \lm{then translate each sub-LF into a natural-language form that is easy for the user to understand (Sub-Question Generation)}, (3) \hs{show natural sub-questions along with intermediate answers to the user and enable them to give feedback for each of sub-questions in turn,} (4) utilize human feedback at each specific turn, along with the contextual information so far, to correct the current sub-LF (Parse Correction). 
 
 
 Under this framework, we formally define two core sub-tasks. \textbf{(1) Parse correction with natural language feedback:} \hs{For each user turn,} given the sub-question $q$ provided by the user as feedback and various contexts, a new sub-LF $p$ is generated. \lm{Sub-LFs will be compiled eventually to produce a corrected parse $P$ for the entire question.} \textbf{(2) Sub-question generation:} given a sub-LF $p$ and \hs{various contexts including the original question}, the task is to generate a natural sub-question $q$.
 


In order to build models for both sub-tasks, we construct a dialogue dataset \textsc{INSPIRED}, which will be detailed in Section \ref{dataset_construction}. Meanwhile, as a simplifying assumption, we take gold named entities mentioned in a question as given. Specifically, we replace named entities in an LF with special tokens such as \textsl{\#entityX\#}, where \textsl{X} is a number corresponding to the order in which the entity appears in the LF. After parsing, we replace these tokens with the gold entities. We acknowledge that addressing errors caused by named entity recognition and linking in a real KBQA system is also challenging and leave it as an important piece of future work.



==> preliminaries.tex <==
\section{Overview}
\label{preliminaries}



 In this work, we seek to design an interactive semantic parsing framework to correct initial parses produced by KBQA semantic parsers via \mww{step-by-step} user interaction. Formally, given a complex question, a knowledge base, a predicted parse from a base parser, and natural-language feedback from the user, the goal is to \mww{derive} a corrected parse. Under this framework, we define two core tasks: (1) parse correction with natural language feedback; (2) \mww{generating} a natural-language question from a sub-logical form (sub-question generation).  
 
To construct such a framework, as shown in \lm{Figure~\ref{fig:full_process}}, we (1) first break down the predicted parse and then translate each piece into a natural-language form that is easy for users to understand (i.e., sub-question generation task), (2) construct an interactive platform using ParlAI~\cite{miller2017parlai} to include users in a dialogue, showing translated pieces along with intermediate answers and enabling them to give feedback \lm{for each piece in turn}, (3) utilize human feedback at each specific turn, along with the contextual information so far, to correct the current piece of the parse, (4) finally compile corrected pieces together to generate a more accurate parse for the original complex question. The parse correction task refers to (3) and (4). We compare the corrected parse and the gold parse using an exact-match metric and report the average accuracy across the testing examples. In order to build models for sub-question generation and parse correction, we need to construct a dialogue dataset, which will be detailed in Section \ref{dataset_construction}.

\lm{In this work, we focus on correcting errors in predicates, \mww{filtering conditions and comparatives/superlatives. As a simplifying assumption, we take gold named entities mentioned in a question as given.}
%SPARQL syntax and assume gold named entities mentioned in a question are given. 
Specifically, we replace named entities in a logical form with special tokens such as \textsl{\#entityX\#}, where \textsl{X} is a number corresponding to the order in which the entity appears in the logical form. After parsing, we replace these tokens with the gold entities. We acknowledge that addressing errors caused by named entity recognition and linking in a real KBQA system is also challenging and leave it as an important piece of future work.}




==> tables/ablation.tex <==
\begin{table*}[t!]
\begin{center}
\resizebox{1\linewidth}{!}
{
\begin{tabular}{l|c|c|c||c}
\toprule
 {} & \multicolumn{3}{c||}{\textbf{Input}} & \textbf{Output} \\
 \hline
\textbf{} & \textbf{Current Q} & \textbf{Previous Qs} & \textbf{Previous LFs}  & \textbf{Current LF} \\
\hline
\makecell[c]{Hop1} & \makecell[c]{In what nation can you find\\ the Al Sharqia Governorate?} & None & None & \makecell[c]{<sparql-header-1> ?c \\ns:location.country.administrative\_divisions\\ \#entity1\#} \\
\hline

\makecell[c]{Hop2} & \makecell[c]{What is the official language\\ spoken in the above-named nation?} & \makecell[c]{In what nation can you find\\ the Al Sharqia Governorate} & \makecell[c]{<sparql-header-1> ?c \\ns:location.country.administrative\_divisions\\ \#entity1\#} & ?c ns:location.country.official\_language ?x . \\
\hline
+ No Context     &  \checkmark & & &  \\
+ Previous Qs & \checkmark & \checkmark & & \\
+ Previous LFs & \checkmark & & \checkmark &  \\
+ Previous Qs \& LFs & \checkmark & \checkmark & \checkmark &  \\
\hline
\bottomrule
\end{tabular}
\vspace{-5pt}
}
\caption{Input with varying contexts and outputs for parse correction task. Different parts involved in the input of every variant are concatenated with a separator `</s>'. }
\label{tab:parse_1}

\end{center}
\vspace{-15pt}
\end{table*}





\begin{table*}[t!]
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|c|c|c||c}
\toprule
 {} & \multicolumn{3}{c||}{\textbf{Input}} & \textbf{Output} \\
 \hline
\textbf{} & \textbf{Current LF} & \textbf{Previous LFs} & \textbf{Complex Q}  & \textbf{Current Q} \\
\hline
\makecell[c]{Hop1} & \makecell[c]{<sparql-header-1> ?c \\ns:location.country.administrative\_divisions\\ \textbf{Al Sharqia Governorate}} & None & \makecell[c]{What is the official language\\ of the country that contains\\ Al Sharqia Governorate?} & \makecell[c]{In what nation can you find\\ the Al Sharqia Governorate?} \\
\hline

\makecell[c]{Hop2} &  ?c ns:location.country.official\_language ?x . & \makecell[c]{<sparql-header-1> ?c \\ns:location.country.administrative\_divisions\\ \textbf{Al Sharqia Governorate}} & \makecell[c]{What is the official language\\ of the country that contains\\ Al Sharqia Governorate?} & \makecell[c]{What is the official language\\ spoken in the above-named nation?} \\
\hline
+ No Context     &  \checkmark & & & \\
+ Previous LFs &\checkmark &\checkmark &  & \\
+ Complex Q &\checkmark & & \checkmark & \\
+ Complex Q + Previous LFs &\checkmark &  \checkmark& \checkmark &  \\
\hline
\bottomrule
\end{tabular}
}
\vspace{-5pt}
\caption{Input with varying contexts and outputs for question generation task. Different parts involved in the input of every variant are concatenated with a separator `</s>'.}
\label{tab:parse_1}
\end{center}
\vspace{-15pt}
\end{table*}

==> tables/multi_attempt.tex <==
\begin{table}[t!]
\begin{center}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cc}
\toprule
\textbf{Attempt Num} & \textbf{EM} & \textbf{F1} \\
\hline
\textbf{BART-large} & &   \\
1   & 75.1 & 75.7 \\
2  & 78.7 & 79.9 \\
3  & \textbf{79.0} & \textbf{80.1} \\ 
\bottomrule
\end{tabular}}
\vspace{-5pt}
\caption{Performance of BART-large after multiple attempts of parse correction.}
\label{tab:multi}
\end{center}
\vspace{-15pt}
\end{table}

==> tables/simulation.tex <==


\begin{table}[t!]
\begin{center}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|cc|cc}
\toprule
\textbf{Models} & \textbf{EM} & \textbf{EM*} & \textbf{F1} & \textbf{F1*} \\
\hline
BART-large & 60.9 & \textbf{75.1} & 65.8 & \textbf{75.7} \\
\hline
QGG & - & - & 49.0 & \textbf{56.5} \\
% QGG$_{real}$ & - & - & 38.7 & \textbf{45.7}\\
\bottomrule
\end{tabular}}
\vspace{-5pt}
\caption{Performance of two types of semantic parsers after parse correction through simulation process. * denotes the performance after correction. BART-large \cite{lewis2020bart}, QGG~\cite{lan:acl2020}.}
\label{tab:simulation}
\end{center}
\vspace{-15pt}
\end{table}

